Sample Complexity Bounds on Differentially Private Learning via Communication Complexity

In this work we analyze the sample complexity of classification by differentially private algorithms. Differential privacy is a strong and well-studied notion of privacy introduced by Dwork et al. (2006) that ensures that the output of an algorithm leaks little information about the data point provided by any of the participating individuals. Sample complexity of private PAC and agnostic learning was studied in a number of prior works starting with (Kasiviswanathan et al., 2008) but a number of basic questions still remain open, most notably whether learning with privacy requires more samples than learning without privacy. We show that the sample complexity of learning with (pure) differential privacy can be arbitrarily higher than the sample complexity of learning without the privacy constraint or the sample complexity of learning with approximate differential privacy. Our second contribution and the main tool is an equivalence between the sample complexity of (pure) differentially private learning of a concept class $C$ (or $SCDP(C)$) and the randomized one-way communication complexity of the evaluation problem for concepts from $C$. Using this equivalence we prove the following bounds: 1. $SCDP(C) = \Omega(LDim(C))$, where $LDim(C)$ is the Littlestone's (1987) dimension characterizing the number of mistakes in the online-mistake-bound learning model. Known bounds on $LDim(C)$ then imply that $SCDP(C)$ can be much higher than the VC-dimension of $C$. 2. For any $t$, there exists a class $C$ such that $LDim(C)=2$ but $SCDP(C) \geq t$. 3. For any $t$, there exists a class $C$ such that the sample complexity of (pure) $\alpha$-differentially private PAC learning is $\Omega(t/\alpha)$ but the sample complexity of the relaxed $(\alpha,\beta)$-differentially private PAC learning is $O(\log(1/\beta)/\alpha)$. This resolves an open problem of Beimel et al. (2013b).

==> ppac-cc-dist.tex <==
We also study distribution-specific versions of the deterministic and
probabilistic representation dimensions.  Let $\calC$ be a concept
class of functions $X \rightarrow \zo$ and $H$ be a family of functions
$X \rightarrow \zo$.

Similar to before, we say that $H$ $\eps$-deterministically represents a
concept class $\calC$ with respect to a distribution $\calD$ if for
every $f \in \calC$, there exists $h \in H$ such that $\Pr_{x \drawnr
  \calD}[f(x) \neq h(x)] \leq \eps$.

Let $\calH$ be a distribution over families of functions, then we say
$\calH$ $(\eps, \delta)$-probabilistically represents $\calC$ with
respect to a distribution $\calD$ if for every $f \in \calC$, with
probability at least $1-\delta$ over $H \drawnr \calH$, there exists
$h \in H$ such that $\Pr_{x \drawnr \calD}[f(x) \neq h(x)] \leq \eps$.

\begin{definition}
  Define:
  \begin{align*}
    \DRDim^\calD_\eps(\calC) & = \min \left\{ \log |H| : \text{$H$
        $\eps$-deterministically represents $\calC$ w.r.t. $\calD$}
    \right\} \\
    \PRDim^\calD_{\eps,\delta}(\calC) & = \min \left\{ \max_{H \in
        \supp(\calH)} \log |H| :  \text{$\calH$
        $(\eps,\delta)$-deterministically represents $\calC$ w.r.t.
        $\calD$} \right\}
  \end{align*}
\end{definition}

Note that $\DRDim^\calD_\eps(\calC)$ is just the logarithm of the size
of the smallest $\eps$-covering of $\calC$ with respect to the metric
induced by $\calD$, which is often called the \emph{metric entropy} in
the learning and approximation literature.

It is clear for all $\eps,\delta > 0$, $\calC$, $\calD$ that:
\begin{equation}
  \label{eq:hpoiahsga}
  \PRDim^\calD_{\eps,\delta}(\calC) \leq \PRDim^\calD_{\eps,0}(\calC)
  = \DRDim^\calD_{\eps}(\calC)
\end{equation}

In fact, the converse also holds.
\begin{theorem}
  \label{thm:distreverse}
  For all $\eps \in (0, 1/2),\delta \in (0, 1)$, and all $\calC$,
  $\calD$ it holds that:
  $$\PRDim^\calD_{\frac{\eps}{2},\delta}(\calC) \geq \DRDim^\calD_{\eps}(\calC)
  - \log(\tfrac{1}{1-\delta})$$
\end{theorem}
\begin{proof}
  $\DRDim^\calD_{\eps}(\calC)$ is at most the logarithm of the size of
  the maximal $\eps$-packing in $\calC$ with respect to the metric
  $d(f, g) = \Pr_{x \drawnr \calD}[f(x) \neq g(x)]$.  This is because
  any maximal packing $P$ is also an $\eps$-covering (otherwise there
  is an uncovered point that we could add to the packing,
  contradicting maximality).

  Let $H$ be a minimal $\eps$-covering, \ie attaining
  $\DRDim^\calD_\eps(\calC)$.  Let $P$ be a maximal packing of size
  $|P| \geq |H|$.  Let $\calH'$ be any $\frac{\eps}{2}$-probabilistic
  representation of $\calC$ w.r.t. $\calD$.  For any $f \in \calC$,
  define $E_f$ to be the event that $H' \drawnr \calH'$ contains some
  $h$ such that $\Pr_{x \drawnr \calD}[f(x) \neq h(x)] \leq \eps$.  By
  definition of $\calH'$ we know that $\Pr_{\calH'}[E_f] \geq 1 -
  \delta$.  We also know that since $P$ is a $\eps$-packing, for every
  $H' \in \supp(\calH'), h \in H'$ there is at most one $f \in P$ such
  that $\Pr_{x \drawnr \calD}[f(x) \neq h(x)] \leq \eps/2$.  Therefore
  we have that:
  $$\Exp_{H' \drawnr \calH'}[|H'|] \geq \Exp_{H' \drawnr
    \calH'}\left[\sum_{f \in P} E_f \right] \geq (1-\delta)|P| \geq (1-\delta)|H|$$
  Therefore it holds that
  $\PRDim^\calD_{\frac{\eps}{2},\delta}(\calC) \geq \DRDim^\calD_{\eps}(\calC)
  - \log(\tfrac{1}{1-\delta})$.
\end{proof}

\subsection{Communication complexity characterizations}

As with the distribution-independent notions, it is possible to
characterize the distribution-specific dimensions in terms of
communication protocols.  The correct notion in this case is a hybrid
worst-case/average-case notion, where Alice's input $f \in \calC$ is
worst-case but Bob's input $x \in X$ is drawn according to some
distribution $\calD$, and Bob wishes to evaluate $f(x)$.  To simplify
the presentation, we define the following only in this specific
context.

\begin{definition}
  Let $\Rand^{\rightarrow}_\eps(\Eval_\calC; \calD)$ be the cost of
  the best one-way protocol $\pi$ from Alice to Bob such that for all
  $f \in \calC$ it holds that
  $$\Pr_{x \drawnr \calD, \pi}[\text{Bob outputs }f(x)] \geq 1 - \eps$$
  Let $\Rand^{\rightarrow,\pub}_\eps(\Eval_\calC; \calD)$ be the same
  but where we restrict to public-coin protocols.
\end{definition}

\begin{theorem}
  \label{thm:distcc}
  For every $\calD, \calC$ and every $\eps \in (0, 1/2), \delta \in
  (0, 1)$
  it holds that
  \begin{eqnarray}
    \Rand^{\rightarrow,\pub}_{\eps+\delta}(\Eval_\calC; \calD) & \leq
    \PRDim_{\eps,\delta}^\calD(\calC) & \leq
    \Rand^{\rightarrow,\pub}_{\eps\delta}(\Eval_\calC;
    \calD)   \label{eq:aposdighapbn} \\
    \Rand^{\rightarrow}_{\eps}(\Eval_\calC; \calD) & \leq
    \DRDim_{\eps}^\calD(\calC) & \leq
    \Rand^{\rightarrow}_{\eps/2}(\Eval_\calC;\calD)
    \label{eq:anpbzodifhbpa}
  \end{eqnarray}
\end{theorem}
\begin{proof}
  \begin{itemize}
  \item For the left inequality of \autoref{eq:aposdighapbn}, consider
    $\calH$ attaining $\PRDim^\calD_{\eps,\delta}(\calC)$.  We may
    construct the protocol where first using public coins the parties
    sample $H \drawnr \calH$, then Alice sends $h \in H$ that is
    $\eps$-close to her input $f$ if it exists, otherwise she sends an
    arbitrary element of $H$.  Bob then outputs $h(x)$.  This achieves
    error at most $\eps + \delta$ and has communication $\max_{H \in
      \supp(\calH)} \log |H|$.
  \item For the right inequality of \autoref{eq:aposdighapbn},
    consider the public-coin protocol $\pi$ attaining
    $\Rand^{\rightarrow,\pub}_{\eps\delta}(\Eval_\calC; \calD)$.  Let
    $r$ denote the public coins of $\pi$ and let $H_r$ denote the
    family of $2^{\CC(\pi)}$ functions that Bob can compute (one for
    each possible Alice message).  Then $\calH$ consists of sampling
    $r$ uniformly and outputting $H_r$.  Clearly $\max_{H \in
      \supp(\calH)} \log |H| \leq \CC(\pi)$.  We claim that $\calH$
    $(\eps, \delta)$-probabilistically represents $\calC$.  For
    otherwise, if there existed $f \in \calC$ such that with
    probability $> \delta$ we sample $H_r$ such that $\forall h \in
    H_r$, $\Pr_{x \drawnr \calD}[f(x) = h(x)] > \eps$, then this
    implies $\pi$ has error $> \eps \delta$, a contradiction.
  \item For the left inequality of \autoref{eq:anpbzodifhbpa},
    consider $H$ attaining $\DRDim_{\eps}^\calD(\calC)$.  The
    deterministic protocol where Alice chooses the $h \in H$ closest
    to her input $f$ and sends it to Bob achieves error $\eps$ and has
    communication $\log |H|$.
  \item For the right inequality of \autoref{eq:anpbzodifhbpa},
    consider the optimal protocol $\pi$ attaining
    $\Rand^{\rightarrow}_{\eps\delta}(\Eval_\calC; \calD)$.  For each
    possible Alice message $\sigma$, consider the randomized function
    $g_\sigma$ that Bob computes (using private coins $r_B$) and define
    $h_\sigma$ as follows:
    $$h_\sigma(x) = \mathrm{majority}_{r_B} \{ g_\sigma(x; r_B) \}$$
    We claim that $$H = \{h_\sigma \mid \sigma \in \zo^{\CC(\pi)}
    \}$$ $\eps$-deterministically represents $\calC$.  For any $f \in
    \calC$, by the error guarantee on $\pi$ there must exist $\sigma
    \in \zo^{\CC(\pi)}$ such that:
    $$\Pr_{x \drawnr \calD, r_B}[g_\sigma(x; r_B) = f(x)] \geq 1 - \eps/2$$
    We claim that the corresponding $h_\sigma$ satisfies
    $$\Pr_{x \drawnr \calD}[h_\sigma(x) = f(x)] \geq 1 - \eps$$
    This is because the probability of a bad $x$ (one where the
    majority of $g_\sigma(x; r_B)$ is wrong) must be bounded by
    $\eps$, and for the good $x$ it holds that $h_\sigma(x) = f(x)$.
  \end{itemize}
\end{proof}

\subsection{Relationship to VC dimension}

It is known that the maximal metric entropy over all possible input
distributions is equivalent to the VC-dimension up to constants
\cite{Kulkarni:89, Dudley:78}.  In our language, this means
\begin{theorem}[\cite{Kulkarni:89, Dudley:78}]
  \label{thm:metricentropy}
  For any $\eps \in (0, 1/4)$ and any $\calD, \calC$, it holds that:
  $$
  \Omega((1-4\eps)^2 \VCDim(\calC)) \leq \max_\calD
  \DRDim^\calD_\eps(\calC) \leq O\left(\log (\tfrac{1}{\eps})
  \VCDim(\calC)\right)
  $$
\end{theorem}

Due to \autoref{thm:distreverse} and \autoref{eq:hpoiahsga}, the same
holds for $\PRDim$:
% Next we show that the maximal $\PRDim^\calD$ is also equivalent to the
% VC-dimension.  Namely, it holds that
\begin{equation}
  \label{eq:apdobiahpd}
  \Omega((1-4\eps)^2\VCDim(\calC)) \leq \max_{\calD}
  \PRDim^\calD_{\eps,\delta}(\calC) \leq  O(\log(\tfrac{1}{\eps})
  \VCDim(\calC))
\end{equation}
% In light of \autoref{eq:hpoiahsga} and \autoref{thm:metricentropy} it
% only remains to prove the first inequality.

% \begin{theorem}
%   $$\max_{\calD} \PRDim^\calD_{\eps,\delta}(\calC)
%   \geq \Omega((1-\eps-\delta)^2\VCDim(\calC))$$
% \end{theorem}
% \begin{proof}
%   Define the maximal complexity under product distributions as follows
%   $$
%   \Rand^{\rightarrow,\times}_\eps(\calC) \triangleq \max_{\calF, \calD}
%   \Dist^{\rightarrow}_\eps(\Eval_\calC; \calF \times \calD)
%   $$
%   Here the maximum is over distributions $\calF$ over $\calC$ and
%   distributions $\calD$ over the input space.  Recall from
%   \cite{KremerNR:99} that
%   \begin{theorem}[\cite{KremerNR:99}]
%     \label{thm:vc}
%     For every $\calC$ and $\eps \in (0, 1/2)$, it holds that
%     $\Rand_{\eps}^{\rightarrow, \times}(\Eval_\calC) \geq
%     \Omega((1-\eps)^2 \VCDim(\calC))$.
%   \end{theorem}
%   Therefore, it suffices to prove
%   \begin{equation}
%     \label{eq:snpodbihags}
%     \max_{\calD} \PRDim^\calD_{\eps,\delta}(\calC) \geq
%     \Rand_{\eps+\delta}^{\rightarrow, \times}(\Eval_\calC)
%   \end{equation}

%   As a direct consequence of \autoref{eq:aposdighapbn}, for any
%   $\calD$ and any distribution $\calF$ over $\calC$, it holds that:
%   $$\Dist^{\rightarrow}_{\eps+\delta}(\Eval_\calC; \calF \times
%   \calD) \leq \Rand^{\rightarrow,\pub}_{\eps+\delta}(\Eval_\calC; \calD)
%   \leq \PRDim_{\eps,\delta}^\calD(\calC) $$
%   Therefore, taking the maximum over all $\calD, \calF$, we obtain:
%   $$ \max_\calD \PRDim^\calD_{\eps,\delta}(\calC) \geq \max_{\calD,
%     \calF}   \Dist_{\eps+\delta}^{\rightarrow}(\Eval_\calC; \calF \times
%   \calD) = \Rand_{\eps+\delta}^{\rightarrow, \times}(\Eval_\calC)$$
% \end{proof}

  %% To show the right inequality of \autoref{eq:snpodbihags} we use
  %% min-max.  Let $c = \Rand^{\rightarrow,\times}_{\eps\delta}(\calC)$.
  %% Then \emph{w.l.o.g.} for every $\calF$ over the concept class
  %% $\calC$ and $\calD$ over the input space $X$, there exists a
  %% deterministic one-way protocol where Alice sends $c$ bits achieving
  %% average error $\leq \eps\delta$.

  %% For any fixed $\calD$, consider the following zero-sum two-player
  %% game $G_\calD$: the row player picks $H$ a set of $2^c$ functions
  %% mapping $X \rightarrow \zo$, the column player picks $f \in \calC$.
  %% The column player wishes maximize and the row player wishes to
  %% minimize the payoff
  %% $$p(f, H) = \begin{cases}
  %%   0 & \exists h \in H \text{s.t.} \Pr_{x \drawnr \calD}[h(x) \neq
  %%   f(x)] \leq \eps \\
  %%   1 & \text{ otherwise}
  %% \end{cases}
  %% $$
  %% Let $V(G_\calD)$ be the value of the game.  By min-max, we know that
  %% $$V(G_\calD) = \min_\calH \max_f \Exp_{H \drawnr \calH}[p(f, H)] =
  %% \max_\calF \min_H \Exp_{f \drawnr \calF}[p(f, H)]$$ %
  %% By hypothesis, we know that
  %% $$\max_{\calD} V(G_\calD) = \max_{\calD, \calF} \min_H \Exp_{f
  %%   \drawnr \calF}[p(f, H)] \leq \delta$$ %
  %% This holds because for any $\calD, \calF$, let $H$ be the set of all
  %% functions Bob can computes (there are $2^c$ such functions,
  %% depending on the message he receives from Alice).  Then $\Exp_{f
  %%   \drawnr \calF}[p(f, H)] \leq \delta$, for otherwise if on a $>
  %% \delta$ fraction of $f \drawnr \calF$ it held that for all $h \in
  %% H$, $\Pr_{x \drawnr \calD}[f(x) \neq h(x)] > \eps$, then the overall
  %% error of the protocol would exceed $\eps \delta$, a contradiction.

  %% By min-max, we therefore have that
  %% $$\max_{\calD} V(G_\calD) = \max_{\calD} \min_{\calH} \max_f \Exp_{H
  %%   \drawnr \calH}[p(f, H)] \leq \delta$$ %
  %% That is, for every $\calD$, there exists $\calH$ such that for every
  %% $f$, with probability $> 1 - \delta$ over $H \drawnr \calH$ there
  %% exists $h \in H$ such that $\Pr_{x \drawnr \calD}[h(x) \neq f(x)]
  %% \leq \eps$.
  %% But this means that $\calH$ $(\eps,\delta)$-probabilistically
  %% represents $\calC$ w.r.t. $\calD$.  Also, by definition $\max_{H \in
  %%   \calH} \log |H| = c$.  Therefore $\max_{\calD}
  %% \PRDim^\calD_{\eps,\delta}(\calC) \leq c$ proving the right
  %% inequality of \autoref{eq:snpodbihags}.

\subsection{Proper notions}

\newcommand{\prop}{\mathsf{prop}}

It is well-known for metric entropy that one can restrict to
representations that are themselves subsets of the concept class
without losing much in the parameters, \ie one can restrict attention
to \emph{proper} notions. % We reprove this here for the sake of
% completeness and also extend it to the probabilistic notion
% $\PRDim^\calD$.
Let a superscript $\prop$ on $\DRDim$ or $\PRDim$
denote ``proper'' versions of those notions, where we take the
minimum over $H$ or $\calH$ only over subsets of $\calC$ rather
than arbitrary subsets of functions $X \dans \zo$.
\begin{proposition}
  For all $\eps \in (0, 1/2), \delta > 0$ it holds that:
  \begin{eqnarray*}
    \DRDim^\calD_\eps(\calC) & \leq
    \DRDim^{\calD,\prop}_{\eps}(\calC) & \leq
    \DRDim^\calD_{\eps/2} (\calC) \\
    \PRDim^\calD_{\eps,\delta}(\calC) & \leq
    \PRDim^{\calD,\prop}_{\eps,\delta}(\calC) & \leq
    \PRDim^\calD_{\eps/2,\delta} (\calC) \\
  \end{eqnarray*}
\end{proposition}
\noindent The proof for $\DRDim$ is well-known and essentially uses
the fact that if $H$ is an $\eps$-representation of $C$, then $C$ is
also an $\eps$-representation of $H$. The proof for $\PRDim$ can be
argued directly in a similar way, or can be derived (with slightly
worse bounds) from the $\DRDim$ case by using
\autoref{thm:distreverse}.

% \begin{proof}
%   The first inequality in each line is obvious since we are taking a
%   minimum over a more restricted set.  Thus we only prove the second
%   inequality in each line.

%   \textbf{Proof that $\DRDim^{\calD,\prop}_{\eps}(\calC)
%     \leq \DRDim^\calD_{\eps/2}(\calC)$:} fix the (improper) $H$ that
%   $\eps/2$-deterministically represents $\calC$ w.r.t. $\calD$ and
%   achieves $\log |H| = \DRDim^\calD_{\eps/2}(\calC)$.

%   We claim that $H$ is $\frac{\eps}{2}$-deterministically represented by
%   $\calC$ w.r.t. $\calD$.  This holds because if there existed some
%   $h_0$ that is $\frac{\eps}{2}$-far from every $f \in \calC$ w.r.t. $\calD$,
%   then the set $H \setminus \{h_0\}$ would also
%   $\frac{\eps}{2}$-deterministically represent $\calC$ w.r.t. $\calD$,
%   contradicting the minimality of $H$.

%   For any $H$ that is $\frac{\eps}{2}$-deterministically represented by
%   $\calC$ w.r.t. $\calD$, define $\rho(H)$ as follows: for every $h
%   \in H$, take an arbitrary $f \in \calC$ such that $\Pr_{x \drawnr
%     \calD}[f(x) \neq h(x)] \leq \frac{\eps}{2}$ (such an $f$ is guaranteed to
%   exist).  Thus we have $|\rho(H)| = |H|$ and $\rho(H)$
%   $\frac{\eps}{2}$-deterministically represents $H$.  We conclude that
%   $\rho(H)$ $\eps$-deterministically represents $\calC$.

%   \textbf{Proof that $\PRDim^{\calD,\prop}_{\eps,\delta}(\calC) \leq
%     \PRDim^\calD_{\frac{\eps}{2}}(\calC)$:} similarly, let $\calH$ be the
%   minimal improper probabilistic representation attaining
%   $\PRDim^{\calD,\prop}_{\eps,\delta}(\calC)$.  We can assume without
%   loss of generality that $\calC$ $\frac{\eps}{2}$-deterministically
%   represents \emph{every} $H \in \supp(\calH)$.  For otherwise if
%   there exists $H \in \supp(\calH)$ and $h_0 \in H$ that is
%   $\frac{\eps}{2}$-far from every $f \in \calC$ w.r.t. $\calD$, then we can
%   modify $\calH$ by replacing $H$ with $H \setminus \{h_0\}$; this
%   would still $\frac{\eps}{2}$-probabilistically represent $\calC$, and this
%   does not increase its size.

%   Build $\rho(\calH)$ from $\calH$ as follows: sample $H \drawnr
%   \calH$ and output $\rho(H)$.  By construction, it holds that
%   $\max_{H \in \supp(\rho(\calH))} \log |H| = \max_{H \in \supp(\calH)
%   } \log |H|$.

%   Finally, observe that for every $f \in \calC$ it holds that with
%   probability $1-\delta$, we sample $H \drawnr \calH$ containing $h$
%   that is $\frac{\eps}{2}$-close to $f$ w.r.t. $\calD$.  Then by the triangle
%   inequality, we know that $\rho(H)$ contains $h'$ that is
%   $\eps$-close to $f$ w.r.t. $\calD$.  This implies $\rho(\calH)$
%   $(\eps,\delta)$-probabilistically represents $\calC$.
% \end{proof}

\subsection{Distribution-specific learning}

We can also consider the question of distribution-specific learning,
where the input distribution is known to the learning algorithm.  The
results in this and the next section are more or less already known,
so for simplicity we restate them for the case where $(\eps, \delta)$
are fixed small constants and provide only proof sketches.

It is known \cite{BenedekI:91} that using $O(\DRDim^\calD(\calC))$ is
necessary and sufficient to learn without privacy.
\cite{BeimelNS:13manu} showed that $O(\VCDim(\calC))$ samples suffice
to learn privately when (an approximation of) $\calD$ is known. Our
result sharpens this even further to $\DRDim^\calD(\calC)$.
\begin{theorem}
  For any $\calC, \calD$ and $\alpha > 0$, $O(\DRDim^\calD(\calC))$
  samples are sufficient to $(\frac{1}{8}, \frac{1}{8})$-learn with
  $\alpha$-differential privacy.
\end{theorem}
\begin{proof}
  Let $H$ be the optimal $\frac{1}{8}$-deterministic representation of
  $\calC$ w.r.t. $\calD$.  Take $O(\DRDim^\calD(\calC))$ samples and
  use the exponential mechanism to sample from $H$ using the quality
  function $q_S(h, f) = \Pr_{x \drawnr S}[f(x) = h(x)]$ and with
  privacy parameter $\alpha$.  Using \autoref{thm:em} and for an
  appropriate choice of constants, it follows that with probability
  $\frac{3}{4}$ the output is has error at most $\frac{1}{4}$.
\end{proof}

Thus, in the case of distribution-specific learning, we can add
privacy \emph{without} any additional cost in terms of sample complexity.

\subsection{Label privacy}

This distribution-specific result can be applied to prove that one can
achieve \emph{label}-differential privacy using $O(\VCDim(\calC))$
samples, \ie where we are only concerned with the privacy of the
labels and not the privacy of the samples themselves.  That is,
$(\alpha, \beta)$-label privacy is defined as in the definition of
differential privacy, except that we \emph{only} consider neighboring
inputs $S, S'$ that differ on one input's label and are identical
everywhere else.

The idea is to first use $O(\VCDim(\calC))$ samples to obtain an
approximation to $\calD$, and then to use the distribution-specific
learning algorithm, which uses $O(\DRDim^\calD(\calC)) =
O(\VCDim(\calC))$ samples.  This was claimed in a manuscript of
\cite{ChaudhuriDKMT:06} and a proof appears in \cite{ChaudhuriHsu:11}
and the idea is similar.
\begin{theorem}[\citep{ChaudhuriDKMT:06, ChaudhuriHsu:11}]
  \label{thm:ppacspecific}
  For any $\calC$ and $\alpha > 0$, $O(\VCDim(\calC))$ samples
  are sufficient to $(\frac{1}{4}, \frac{1}{4})$-learn $\calC$ with
  $\alpha$-differential privacy.
\end{theorem}
\begin{proof}
  Consider the concept class $\calC \oplus \calC = \{ f \oplus g \mid
  f, g \in \calC\}$.  An application of Sauer's lemma shows that
  $\VCDim(\calC \oplus \calC) = O(\VCDim(\calC))$.

  Our algorithm is as follows:
  \begin{enumerate}
  \item Sample $t = O(\VCDim(\calC \oplus \calC))$ samples from
    $\calD$, call this set of samples $S$.
  \item Let $\calD_S$ be the uniform distribution over $S$.  Let $H$
    be the optimal \emph{proper} $\frac{1}{8}$-deterministic representation
    of $\calC$ over $\calD_S$.
  \item \label{item:specific} Use the algorithm of
    \autoref{thm:ppacspecific} to $(\frac{1}{8},
    \frac{1}{8})$-learn $\calC$ with respect to $\calD$ and with
    $\alpha$-differential privacy.  Note that the number of samples
    required is at most
    $$O(\DRDim^{\calD_S,\prop}(\calC)) = O(\DRDim^{\calD_S}(\calC)) =
    O(\VCDim(\calC))$$
    Finally, output this hypothesis.
  \end{enumerate}

  The sample complexity holds by definition.  Label privacy holds
  because we do not use the labels for the first $t$ samples and
  therefore changing those labels has no effect on the output, while
  for samples used in \autoref{item:specific} are protected by
  differential privacy (not just for the labels but even for the
  samples).

  We show that this learner indeed succeeds in producing a good
  hypothesis.  First from standard sample complexity bounds we know
  that for a large enough $t = O(\VCDim(\calC \oplus \calC))$ , with
  probability $7/8$ it holds that for all $f, g \in \calC$:
  $$\left|\Pr_{x \drawnr \calD_S}[f(x) \oplus g(x) = 1] - \Pr_{x \drawnr
    \calD}[f(x) \oplus g(x) = 1] \right| \leq \frac{1}{8}$$
  Or, in other words, for all $f, g \in \calC$:
  \begin{equation}
    \label{eq:apodbfinapdoifnbaohg}
    \left|\Pr_{x \drawnr \calD_S}[f(x) \neq g(x)] - \Pr_{x \drawnr
    \calD}[f(x) \neq g(x)]\right| \leq \frac{1}{8}
  \end{equation}
  Condition on this is indeed being the case.

  Next, we know that with probability $7/8$ the hypothesis $h$
  produced by \autoref{item:specific} satisfies
  \begin{equation}
    \label{eq:aposihgapobnz}
    \Pr_{x \drawnr \calD_S}[f(x) \neq h(x)] \leq \frac{1}{8}
  \end{equation}
  Therefore by a union bound with probability $\frac{3}{4}$ both
  \autoref{eq:apodbfinapdoifnbaohg} and \autoref{eq:aposihgapobnz}
  hold.  In this case, since $h \in \calC$ because the representation
  is proper, \autoref{eq:apodbfinapdoifnbaohg},
  \autoref{eq:aposihgapobnz}, and the triangle inequality imply that
  $$\Pr_{x \drawnr \calD}[f(x) \neq h(x)] \leq \frac{1}{4}$$
  This concludes the proof.
\end{proof}



